AquilaMoE: Efficient Training for MoE Models with Scale-Up and Scale-Out Strategies

In recent years, with the rapid application of large language models across various fields, the scale of these models has gradually increased, and the resources required for their pre-training have grown exponentially. Training an LLM from scratch will cost a lot of computation resources while scaling up from a smaller model is a more efficient approach and has thus attracted significant attention. In this paper, we present AquilaMoE, a cutting-edge bilingual 8*16B Mixture of Experts (MoE) language model that has 8 experts with 16 billion parameters each and is developed using an innovative training methodology called EfficientScale. This approach optimizes performance while minimizing data requirements through a two-stage process. The first stage, termed Scale-Up, initializes the larger model with weights from a pre-trained smaller model, enabling substantial knowledge transfer and continuous pretraining with significantly less data. The second stage, Scale-Out, uses a pre-trained dense model to initialize the MoE experts, further enhancing knowledge transfer and performance. Extensive validation experiments on 1.8B and 7B models compared various initialization schemes, achieving models that maintain and reduce loss during continuous pretraining. Utilizing the optimal scheme, we successfully trained a 16B model and subsequently the 8*16B AquilaMoE model, demonstrating significant improvements in performance and training efficiency.

==> sections/scale-up-exp.tex <==
\subsubsection{Scale-up Validation}
\label{sec:cmp_init}
% 使用不同初始化策略的对比结果及分析 @袁野

\yuanye{Add experiments on depth expansion methods? (stacking vs. interpolation)}

We first compare the FPI and AKI methods based on Aquila2\footnote{https://github.com/FlagAI-Open/Aquila2}. We use a model with 1.3B parameters as the source model, grow the model to 7B size with different methods, and then compare their convergence. We also train a 7B model from scratch for comparison. All these three experiments use the same hyperparameters. \yuanye{Whether to list the hyperparameters or not?} The results are shown in Figure~\ref{fig:fpi-aki-cmp}. The experiments show that with FPI and AKI methods, the model growing from a smaller model will converge much faster than training from scratch. Moreover, we have the same conclusion as the original paper that AKI will perform better.

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
    \includegraphics[width=0.9\linewidth]{figs/cmp-fpi-aki.pdf}
\caption{Comparison of the convergence with FPI and AKI methods. \yuanye{1) refine the figure; 2) refine the wrap location; 3) whether to continue train 7b-fpi?}}
\label{fig:fpi-aki-cmp}
\end{wrapfigure}

